Using RDMA for Lock Management

In this work, we aim to evaluate different Distributed Lock Management service designs with Remote Direct Memory Access (RDMA). In specific, we implement and evaluate the centralized and the RDMA-enabled lock manager designs for fast network settings. Experimental results confirms a couple of hypotheses. First, in the traditional centralized lock manager design, CPU is the bottleneck and bypassing CPU on client-to-server communication using RDMA results in better lock service perofrmance. Second, different lock manager designs with RDMA in consideration result in even better performance; we need to re-design lock management system for RDMA and fast networks.

==> RDMALockManager-CS2270 (2)/server_centric.tex <==
\section{Server Centric Design}
Centralized lock management is one of the simplest design for a lock service that we often encounter in textbooks. This traditional approach can be easily implemented by allowing a single thread to access a shared memory region or a code section, which effectively serialize concurrent requests from multiple clients. In this section, we first describe the architecture and some important implementation details; next we discuss the performance characteristics of the centralized lock manager over a fast Network (i.e., InfiniBand) using TCP/IP sockets and RDMA send/receive verbs.

A centralized lock manager spawns a thread for each incoming client connection; each thread is responsible for the communication between the server and a connecting client. Messaging via TCP/IP sockets incurs context switching overheads and much of CPU cycles are spent on message handling in kernel. In our experiment with 40 clients, each sending 100,000 lock request and release requests, more than 90\% of server CPU cycles were spent on message handling in kernel.

Any requests received by the server are first registered to an array of FIFO queues; each queue holds lock requests for a specific data item. Any access to a queue within the array is protected by a mutex, and clients will block each other only if they are trying to access the same item. When a lock release request is received by a lock holding client, then the corresponding request is popped from the queue after the server acknowledges the release request; the next requests in the queue is granted the lock. Subsequent shared lock requests can be granted together if no client is holding the same lock in the exclusive mode.

TCP/IP blocking read and write are costly, but the burden can be offloaded to network hardware using RDMA send/receive verbs and the saved CPU cycles can be used to process more lock requests; hence, making the lock manager more scalable. 


In Figure~\ref{fig:server_centric_result}(a), the throughput of the traditional design can be improved using RDMA send/receive verbs ($S/R$) and scales with the increasing number of clients. On the other hand, the throughput of the system using TCP/IP socket (TCP) tampers off quickly as the server's CPU is overloaded. With 100 lock items being shared among multiple clients, the server with RDMA tops around at 1.4M locks per second, whereas the one with TCP/IP yields only about 40880 locks per second. Processing a message takes about $10^4$ CPU cycles and assuming forty 3GHz cores, a loose upper bound for the lock throughput is roughly 30M locks per second.

Figure~\ref{fig:server_centric_result}(b) shows how the throughput changes as we vary the contention rate: $CR=1-N_{item}/N_{client}$, where $N_{item}$ is the number of items and $N_{client}$ is the number of clients. Assuming a uniform access pattern for each client, the more clients there are relative to the number of items indicates the higher contention among the clients. Here, the number of clients is fixed at 40.
